SwarmControl: An Automated Distributed Control Framework for Self-Optimizing Drone Networks

Networks of Unmanned Aerial Vehicles (UAVs), composed of hundreds, possibly thousands of highly mobile and wirelessly connected flying drones will play a vital role in future Internet of Things (IoT) and 5G networks. However, how to control UAV networks in an automated and scalable fashion in distributed, interference-prone, and potentially adversarial environments is still an open research problem. This article introduces SwarmControl, a new software-defined control framework for UAV wireless networks based on distributed optimization principles. In essence, SwarmControl provides the Network Operator (NO) with a unified centralized abstraction of the networking and flight control functionalities. High-level control directives are then automatically decomposed and converted into distributed network control actions that are executed through programmable software-radio protocol stacks. SwarmControl (i) constructs a network control problem representation of the directives of the NO; (ii) decomposes it into a set of distributed sub-problems; and (iii) automatically generates numerical solution algorithms to be executed at individual UAVs. We present a prototype of an SDR-based, fully reconfigurable UAV network platform that implements the proposed control framework, based on which we assess the effectiveness and flexibility of SwarmControl with extensive flight experiments. Results indicate that the SwarmControl framework enables swift reconfiguration of the network control functionalities, and it can achieve an average throughput gain of 159% compared to the state-of-the-art solutions.

==> backup_experimental.tex <==

\section{Evaluation}
\label{sec:evaluation}
Following the illustration diagram in Fig. \ref{fig:PPS}, we showcased SwarmControl in the following way: 
(i) The network controller first defines the network behavior through the SwarmControl APIs, selecting among different layer-specific protocols and overall network behavior templates. 
SwarmControl terminal interface runs on a network control host (NCH), which constructs, decomposes and distributes network control problems over the wireless interface to the UAV nodes of the network as explained in Section \ref{sec:ncp} and \ref{sec:distributed}.
(ii) Each single UAV node, locally runs the numerical algorithms in its PPS Control Plane feeding the found solutions to the PPS Data Plane.
The latter is is charge of applying them at
the motion (i.e. UAV's motors) and radio front end (i.e. USRP) over the four Electronic Speed Controllers (ESC) and the USB 3.0 interface, respectively. 
(iii) The motion and the radio front ends distributively implement the overall network behavior selected at the centralized NCH. 

In this work, we operate four distributed optimization algorithms at the Control Plane, namely: TCP congestion window size, network routing table, physical layer transmission power, and hovering location. 
These problems draw key information from the link capacity, SINR, set of neighbors, and neighbors hovering LUTs; and record their numerical solution into transport protocol, routing table, transmission chain and flight control LUTs, respectively.
Thanks to the fast read/write primitive operations of LUTs, the data plane immediately adapts its network and flight control parameters to the fresh numerical solutions, in an on-line fashion. 
Regardless the problem complexity, the distributed optimization algorithms convergence to an optimal solution is guaranteed within a few iterations, until the network state changes. At that point, the search for a new convergence equilibrium restarts, and so on.

\textbf{Experiments} 
SwarmControl has been tested on a plethora of network configurations, varying the number of nodes, number of sessions, topologies, and testing environments; on a fully UAV swarm, and on a hybrid ground/aerial network.
Given the complexity of the network control problem, we tested the effectiveness and flexibility of our new wireless software-defined network control framework in an incremental fashion, showing intermediate step results, to highlight the impact of different features on the overall system performance.
Finally we conclude our performance evaluation with a full aerial deployment where all the functionalities shown in previous experiments are employed.
This section is organized as follows: 
(i) We initially introduce our UAV/SDR network node prototype, then, we highlight our framework optimization effectiveness and flexibility first on (ii) a fully wireless network and then on (iii) a mixed ground/aerial scenario, where SwarmControl is employed to optimize a stand alone wireless infrastructure, and a wireless relay network assisting ground nodes, respectively. 
There we focus on future UAV network applications such as failure recovery and network offloading.
We conclude this section with (iv) flight experiments in an anechoic chamber and Faraday cage facility, comparing obtained results with laboratory evaluation and state of the art optimization frameworks.


\begin{figure}[b]
% \centering
\vspace{-2mm}
\includegraphics[width=0.5\textwidth]{Figures/prototype_2.pdf} \vspace{-5mm}\caption{ \small UAV network node prototype.}\vspace{-0mm}
\label{fig:prototype}
\end{figure}

\begin{figure}[b]
% \centering
\vspace{-2mm}
\includegraphics[width=0.5\textwidth]{Figures/hardware.pdf} \vspace{-5mm}\caption{ \small Prototype hardware design.}\vspace{-0mm}
\label{fig:hardware}
\end{figure}


\subsection{UAV network prototyping}
\label{subsec:prototype}
Despite UAV/SDR are foreseen to shape the future of wireless communications, no product with similar capabilities is on the market yet. 
Therefore we prototype our own UAV/SDR network node.

Each UAV/SDR node is composed of an Intel Aero drone mounting an Ettus Universal Software Radio Peripheral (USRP) B205mini-i Software Defined Radio. 
%Both the UAV and the SDR are battery operated.
%[details about the two tightly communciating boards and the fully wireless charachteristics of the drone - dual band wifi, GPS receiver and SDR driven antenna set]
With a flying time of over 20 minutes, a hub-to-hub diagonal length of 360 mm, a base-to-top height of 222 mm, Intel Aeros offer a high portability and maneuverability. 
The choice for the SDR fell on B205mini-i as they currently are the most compact and lightweight SDR device operating at a low power budget. 
Intel Aero houses a Compute Board providing sufficient computational power to run native Linux Kernel with Ubuntu 16.04. This allows, not only to run all legacy Linux functions, but also to seamlessly run Software Defined Radio development platforms such as Gnuradio. 
Flight management, motors control and sensors fusion are performed on a Pixhawk 4 Flight Controller Unit (FCU), a dedicated board directly interfacing the Computer Board. 
All FCU parameters and commands are accessible via the MAVLink Communication Protocol exposing a UDP port to the OS for remote control and sensor readings.
Differently from legacy UAVs, SwarmControl UAV nodes 
are endowed with a PPS hovering layer PyMavlink-based implementation, allowing each node to be fully autonomous and perform flight control distributively. 
% The Compute Board orchestrates the interaction between the SDR and the FCU.
%[revise: why do we believe that this prototype is a good representation of the future IoT. (we don't want a feature listing here or a product description - especially of features that are not project related e.g. wifi hotspot or remote control)]
%[More on Aero dimension, payload to motivate the use of b205 mini.]
%[technical details on intel aero, ROS, pymavlink, USRP SDR b205mini and network connectivity]
It is worth pointing out that SwarmControl is fully open-source software powered, that the PPS is entirely implemented in Python and runs on native Linux OS, which directly interfaces with the Flight Controller Unit running Pixwawk, and GNURadio, controlling the SDR via USRP hardware driver (UHD); which makes SwarmControl compatible with every MAVLink-based programmable drone interface.
Fig. \ref{fig:prototype} and Fig. \ref{fig:hardware} provide an overview of the prototype of our UAV/SDR network node prototype and its hardware design.
%  which makes SwarmControl compatible with every programmable drone implementation currently available: ROS (Robotic Operating System), DroneKit, PyMavlink. 

\begin{figure*}[t]
\centering
\includegraphics[width=1\textwidth]{Figures/scenarios_avg.pdf} \vspace{-5mm}\caption{ \small Fully UAV network deployments.}\vspace{-5mm}
\label{fig:scenario123}
\end{figure*}

\subsection{Full UAV network}
\label{sec:uav_net}
In this section we test the effectiveness and flexibility of SwarmControl in achieving network performance gains in fully-aerial wireless network scenarios. 
We evaluated the performance of SwarmControl deploying 6 UAV swarms in three different scenarios, namely Scenario 1, 2 and 3 in Fig. \ref{fig:scenario123}. 
Scenario 1, 2, and 3 have been arranged such that the nodes mutually interfere degrading their channel capacity, and that the overall end-to-end network throughput can be expressed as a function of their hovering location, SDR transmit gain, routing table, and TCP congestion window.
The experiment foresees two UAV source nodes opening transport layer sessions with two destinations and injecting traffic over the multi-hop UAV-network.
Scenario 1 and 2 are an dense indoor environment with many obstacles characterized by non-line of sight conditions, high multi-path effect, and high noise power, while Scenario 3 is a characterized by a larger obstacle-free space, low signal refraction and poor multi-path effect.
Specifically, we compare the performances of two different overall network control problems, (1) rate maximization and (2) power consumption minimization with minimum rate constraints, on an eight UAV node swarm; employing three control frameworks, (i) SwarmControl, operating optimization algorithms at the transport, routing, physical and hovering layer of the PPS;
(ii) Best Response, independently optimizing the parameters at the different layers of the PPS with no cross-domain penalization factors; and 
(iii) No Control, not employing any network optimization framework and sticking with initial PPS parameters values.
It is worth pointing out that in all the figures, the showed signal paths represent a single snapshot of the network state, which may evolve throughout the experiment.


\textbf{Achieving optimality gains.}
Three optimization schemes have been tested for two network control problems defined by the NC: 
(i) maximizing the overall sum end-to-end session layer network throughput, and
(ii) minimizing the overall power consumption with minimum session-rate constraints. 
For this and the following experiments the NC selected TCP as a transport layer protocol, Bellman-Ford based routing algorithm, frequency division multiplexing at the MAC and static hovering at the motion layer.

Thanks to SwarmControl, the UAV-network will form, self-organize, and support the injected traffic in a self-optimized fashion toward the defined objective behavior. 
The average performance of SwarmControl with respect to the second best performer for max-performance control problem report overall throughput gains of $52\%$, $90\%$ and $208\%$ for scenarios 1, 2, and 3, respectively, as shown in Fig. \ref{fig:scenario123}.

\begin{figure}[t]
% \centering
\vspace{-5mm}
\includegraphics[width=0.5\textwidth]{Figures/switching_behavior.pdf} \vspace{-8mm}\caption{ \small Switching network behavior.}\vspace{-5mm}
\label{fig:switching_behavior}
\end{figure}



\textbf{Changing the network behavior.}
SwarmControl makes modifying a whole aerial network behavior as simple as inputting few characters into the Control Panel. 
Decomposing and re-distributing the new optimization problems at all the network nodes is handled automatically. The whole procedure takes less that 3 seconds. 
This way it is possible to change the network protocol selection, the network constraints, opting-in standard features, or changing the overall network operational goal.
We operate a change toward a minimization power consumption behavior with minimum session rate requirements and compare network operational points for the two different network control problems for Scenario 1 in Fig. \ref{fig:switching_behavior}.
The nodes' transmission gains and TCP transmission rates reflect the different network control problems for the two behavioral goals, as shown in the lower part of \ref{fig:switching_behavior}.
The top of the Figure shows the measured session rate at the two destinations, reflecting the two dictated network behaviors.

To highlight the two different network operational points, we have terminated session 1 after 180 seconds for both experiments, and observed the different behaviors.
% following the termination of one session.
Despite a general throughput gain following the reduced interference, under Max-log-rate control problem nodes increase the transmission power and TCP rate toward an overall network rate maximization. Contrarily, under Min-power control problem nodes don't, constrained by a power minimization behavioral goal resulting is lower network measured performances.

\subsection{Mixed ground/UAV network.}
\label{sec:mixed_net}
We herein evaluate the opportunities of integrating SwarmControl optimization framework to assist and enhance the performance of a ground wireless infrastructure with a swarm of UAV wireless nodes. 
In this section we first analyze the key principles of a UAV-swarm control framework application to ground/aerial network integration, such as mobility management, failure recovery, and network offloading; then, conclude applying SwarmControl to an emergency relay network for infrastructure recovery in disaster scenarios. 

\begin{figure}[b]
% \centering
\vspace{-0mm}
\includegraphics[width=0.5\textwidth]{Figures/mobility_managament.pdf} \vspace{-8mm}\caption{ \small Mobility deployment.}\vspace{-0mm}
\label{fig:mobility}
\end{figure}

\textbf{Mobility management}
Among all, UAV software-defined networks key feature is mobility management.
SwarmControl distributed optimization algorithms handle mobile nodes in an automatic fashion, calculating optimal network solutions 
% to be adopted by the Data Plane PPS at run-time 
based on the network state variations (SINR, nodes locations, TX Power, etc.) 
We test SwarmControl's mobility management on a 6-UAV swarm in Scenario 4, two of which switch their location every 60 seconds, for a total of 4 times a run. 
We compare the effectiveness of SwarmControl in re-routing the traffic and optimizing network parameters with the dynamic network state to other optimization schemes in Fig. \ref{fig:mobility}.

% The severe location drifting penalizes traditional network optimization methods while SwarmControl is proven to be effective in optimizing the network control objective thanks to the fast interaction between Control Plane and the Data Plane of the newly designed PPS.
Comparing our cross-layer optimization framework with other optimization schemes, we prove the superior effectiveness in handling mobility of SwarmControl, achieving an overall throughput gain of \textbf{XX}.
% The integration of the open source robot operative system in the programmable protocol stack is proven to be a game changer for classic network control problem algorithm execution, overcoming traditional single layer optimization problems. The superior cross-layer optimization strategy, powered by the on-board UAV sensors readings, pushes the network control beyond the limit of traditional network dynamics.
% The SwarmControl's cross-layer optimization problem decomposition approach for UAV networks is proven to overcome traditional schemes, pushing the network control beyond the limits of traditional networks' dynamics.






\begin{figure}[b]
\vspace{-3mm}
\includegraphics[width=0.5\textwidth]{Figures/failure_and_recovery.pdf} \vspace{-5mm}\caption{ \small UAV-aided failure recovery.}\vspace{-0mm}
\label{fig:failure_recovery}
\end{figure}







\textbf{Failure recovery and network offloading.}
% introduction 
Since their first appearance,in the wireless network paradigm, 
UAVs wireless networks have been targeted for rapid ground infrastructure malfunction recovery and stations' traffic offloading \cite{naqvi2018drone}.
% The sensitivity to failure recovery time, as well as on-demand and swift deployment, network reconfiguration, and dominant line-of-sight links  


% netwrok failure
% Node failures in ground wireless networks are normally due to device malfunction or adverse wireless medium conditions, high interference power, or lack of line of sight.
% They might lead to network disconnection and off-periods; and can have serious consequences, from diminished network performance as a whole, to network partitioning.
% offloading
% In traditional wireless networks, bottlenecked nodes often suffer from poor channel conditions due to poor RF signal or long distances from their receivers. 
% The limited total bandwidth available pushes these nodes in high backlogged traffic state which evolves in a fundamental performance bottleneck for the overall network, especially for the hotspot period where the bottleneck node is heavily loaded.
% UAVs for this purpose
% There have been efforts on utilizing autonomous unmanned terrestrial or aerial vehicles to overcome network failure , as well a network offload \cite{naqvi2018drone}. 
% While a network node failure rewards the UAV-aided recovery due to sensitivity to the recovery time, the offloading issue for terrestrial stations can be partly addressed via existing technologies such as Wi-Fi offloading [XX] or small cell [XX], among others. 
% However, these solutions can be pricey, require redundant hardware infrastructure deployment and inadequate for highly variable traffic scenarios.
% Therefore, UAV-aided ground offloading offers promising advantages compared to the conventional network overhead, such as on-demand and swift deployment, network reconfiguration, and dominant line-of-sight links  \cite{wu2019fundamental}.
% SwarmControl for network failure and offloading
We case study the use of SwarmControl for network failure recovery and ground infrastructure offloading, with the aim of improving overall network performances. 
We tested the network recovery and network offloading performances in Scenario 5 (Fig. \ref{fig:failure_recovery}) and Scenario 6 \ref{fig:offloading}), where a set of UAV wireless nodes are employed to overcome a ground node failure and assist an overloaded ground network, respectively.


Fig. \ref{fig:failure_recovery} presents the benefit of UAV-aided ground network recovery where a two-hop wireless ground network failure is aided by a UAV node (Scenario 5).

SwarmControl powered UAV-aided failure recovery rapidly recovers the failed network, preventing network isolation and ensuring minimal application throughput drop over the recovery period ( Fig. \ref{fig:failure_recovery}). 
SwarmControl employed, in this case, a Max-performance control problem to guarantee no performance drops during the assistance phase and rapidly re-routed the backlogged data though UAV A thanks to the wireless flexibility provided by the reconfigurable PPS.


% Given the inflexibility of the ground infrastructure in recovering to failure the UAV node assistance is crucial in quickly and effectively reroute the traffic and recover the network session, possible thanks to the wireless flexibility provided by the reconfigurable PPS.

We showcase the effectiveness of our framework in assisting an overloaded portion of a ground infrastructure toward congestion relief and higher overall network throughput, in Scenario 6 (Fig. \ref{fig:offloading}).
The shown results highlight the performance gain following the offloading of the ground relay congested by the two traffic flows.
SwarmControl network assistance employed two UAVs running a Max-performance control problem in offloading the ground network infrastructure, achieving an average \textbf{XX} throughput gain over ten 4-minute long runs.

\begin{figure}[b]
% \centering
\vspace{-0mm}
\includegraphics[width=0.5\textwidth]{Figures/offloading.pdf} \vspace{-5mm}\caption{ \small UAV-aided offloading.}\vspace{-0mm}
\label{fig:offloading}
\end{figure}

\begin{figure*}[t]
\centering
\vspace{-5mm}
\includegraphics[width=1\textwidth]{Figures/relay_network.pdf}
\vspace{-5mm}\caption{ \small Relay network behavior for two different control problems.}\vspace{-5mm}
\label{fig:relay}
\end{figure*}

\textbf{UAV relay network.}
Some particularly adverse network scenarios requires more than node failure recovery or simple network offloading. 
We pushed the application of UAV networks beyond the scope of network assistance to realize the first wireless software-defined UAV-network for disaster recovery and emergency scenarios.
We tested the effectiveness of SwarmControl on a 6-UAV wireless network, recovering and optimizing the network performances of a disrupted ground infrastructure. 

Scenario 7 in Fig. \ref{fig:relay_network} presents two ground nodes unable to communicate following a network infrastructure collapse, assisted by 6-UAV swarm employing SwarmControl for post disaster infrastructure recovery. 
Beyond recovering the collapsed ground infrastructure, SwarmControl proposes as software controllable framework for distributed UAV emergency networks, allowing not only to re-link ground network sessions in disaster scenarios, but to dictate the network behaviour of the resulting compound infrastructure. 

Changing the overall behavior for recovery UAV-networks, such as maximizing network throughput, or minimizing network power consumption, can be extremely important to select the best operational mode over time, depending on communication criticality, expected recovery time, number of users, coverage area, and traffic load, among others.
Fig. \ref{fig:relay_network} illustrates the relay UAV-network performance for two different control problems, namely Max-log-rate and Min-power. 
The bottom of the figure presents the network operational points on a selected run, showing the relay network single nodes' forwarding rates achieving optimal traffic distribution across the network.
The top part shows the measured application layer recovered throughput at the destination for a single realization and ten 4-minute long runs average.

\begin{figure}[b]
% \centering
\vspace{-5mm}
\includegraphics[width=0.38\textwidth]{Figures/KRI_chamber.png} \vspace{-2mm}\caption{ \small Indoor facility 3-D section model.}\vspace{-0mm}
\label{fig:chamber_section}
\end{figure}





\subsection{SDN in the Sky}
\label{sec:sky}
We conclude this session testing SwarmControl performance on a full 8-UAV wireless network aerial swarm.
We herein evaluate the effectiveness and flexibility of SwarmControl distributed optimization operating at all the layers of the PPS: hovering layer, physical layer, routing layer, and transport layer. 
The resulting network state is determined by the compound effect of four different numerical solution algorithms, making individual contribution on the performance metrics hard to isolate.

We performed extensive flight experiments in an flying indoor facility, featuring anhecoic chamber and Faraday cage properties.
The facility is a 50’x50’x22’ chamber, entirely outdoor and indoor shielded, featuring a 5-wall internal foam coating for total RF signal absorption from 300MHz to 18GHz. 
Despite the absorbing walls and the Faraday cage set ideal conditions for radio transmission, this scenario is not favorable to UAV hovering operations. 
The absence of GPS signal and the poor Earth magnetic field pose severe challenges to distributed flight coordination. 
However, the on-board additional high fps cameras and sonar,  mitigate the absence of universal reference signals.
[pointing out how hard is to have a large set of experiments for battery powered devices].
As for other experiments, two network nodes open a transport layer session toward two destinations, while the rest of the network is to support multi-hop wireless transmission as effectively as possible. We keep all the sources and destinations fixed in "hold" mode, while we let the other nodes free to hover around.
\begin{figure}[b]
% \centering
\vspace{-5mm}
\includegraphics[width=0.5\textwidth]{Figures/chamber_snapshot.pdf} \vspace{-5mm}\caption{ \small Indoor flight snapshot.}\vspace{-5mm}
\label{fig:chamber_flight}
\end{figure}

\begin{figure*}[t]
\centering
\vspace{-5mm}
\includegraphics[width=1.0\textwidth]{Figures/chamber_mobility.pdf} \vspace{-5mm}\caption{ \small Indoor flight experiments.}\vspace{-5mm}
\label{fig:chamber_experiments}
\end{figure*}

\begin{figure}[t]
\vspace{-5mm}
\includegraphics[width=0.5\textwidth]{Figures/chamber_average.pdf} \vspace{-5mm}\caption{ \small Average framework performances in flight experiments.}\vspace{-5mm}
\label{fig:chamber_average}
\end{figure}

Despite the singular contribution of each optimization algorithm is hard to isolate, we like to highlight, on a single realization, the hoovering numerical solution algorithm and the resulting network performance for two network deployments in Fig. \ref{fig:chamber_experiments}.
The right parts of the figure illustrates drone hovering movements over time, dictated by the optimal hoovering location numerical solution algorithm running at the SwarmControl PPS. 
The convergent solution reflects the search of the UAVs optimal location in terms of channel SINR, pushing the relays apart to reduce mutual interference and improve the overall network capacity. 
Comparing the right and the left part of the figure, showing the measured network throughput, it is possible to intuit the hovering optimal solution algorithm impact on the network performance.








% average results
We extensively evaluate SwarmControl performance over the two network deployment scenarios comparing our framework with three optimization schemes:
Best Response (BR), 
No Control (NC), and 
WNOS \cite{guan2018wnos}.
WNOS is a recently developed wireless operating system for infrastructure-less ad-hoc wireless networks, whose open-source code we employed and implemented for our testing experiments. 
% [XX salvo XX - quick overview of WNOS and how we implemented it thank to the open source software]

We obtained an average throughput gain of $87\%$ and $231\%$ on the second the best framework over ten 2-minute long experiment runs.
The performance of SwarmControl are highlighted in Fig. \ref{fig:chamber_average}. 


==> backup_intro.tex <==
\section{Introduction}
\label{sec:introduction}
% \begin{itemize}
% \item Brief intro on drones, 5G, IoT ...

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \textbf{AVAILABILITY OF PROGRAMMABLE SMALL FORM FACTOR UAVs}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The future of radio access networks is soon expected to support up to a 1000-fold increase in traffic volume and 100 billion ubiquitously connected wireless devices, all with heterogeneous requirements in data processing, battery lifetime, transmission range, and latency.%,  among others. 
This will exert pressure on the current infrastructure with high capacity and scalability demands.
% IoT 5G
%THE landscape of future fifth generation (5G) radio access networks is expected to seamlessly and ubiquitously connect everything, and support at least 1000-fold traffic vol- umes, 100 billion connected wireless devices, and diversified requirements on reliability, latency, battery lifetime, etc, as opposed to current fourth generation (4G) cellular networks.  
%Nowadays, the popularity of the Internet of Things (IoT) has triggered a surge in the number of mobile data traffic for upcoming 5G and beyond 5G (B5G) wireless networks. 
%In accordance with the latest report [1], the global mobile traffic will reach 1 zettabyte/mo until 2028. This will lead the current infrastructure facing great capacity demands and also impose a heavy burden on the telecom operators in terms of increased capital investments and operational costs.
To cope with these issues, intelligent Unmanned Aerial Vehicles (UAVs, or drones) have been considered as a promising technology to facilitate the current infrastructure toward the future of wireless networks.
% Over the next decades, embedded vision systems will be- come part of an increasing number of applications that in- clude autonomous or semi-autonomous vehicles, consumer electronics (cameras and mobile phones), and toys. Because of their limited payload capacity and energy capacity, toys, micro-UAVs, and small domestic robots cannot use active imaging sensors and must rely on passive cameras and vi- sion for navigation, obstacle avoidance, and object/target recognition.
The miniaturization of Unmanned Aerial Vehicles could benefit from 
the technological advances in multi-core processors and low-power embedded vision systems for smart-phones.
The new available hardware, that provided high computational resources at a low power budget and low weight, helped turning programmable small form factor UAVs into commodity off-the-shelf products.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \textbf{APPLICATIONS ENABLES - CIVIL / MILITARY}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% use of drones general
UAVs are autonomous aircrafts, that have been used mainly in military applications for many years such as battlefield inspection, geographic mapping of dangerous terrains, border control, and aerial surveillance.
% target tracking, tactical reconnaissance, search and rescue, monitoring of high-tension power lines, photogrammetry and remote sensing.
They have recently got more and more involved by public and civil organizations, as well as companies and individuals in diverse fields, which inspired the 5G revolution.
Non-military applications include provisioned services, precision agriculture, emergency response services, environmental monitoring, and delivery of goods. 

For instance, Soldiers in the U.S. Army will be equipped with nano drones 
% to assist soldiers who do not have an aerial support or satellite connection 
to gain insights about their surroundings \cite{nano_drones}.
At least 30 military and government agencies in China have strengthened their surveillance network with small drones resembling birds
% In the past few years, at least 30 military and government agencies have deployed these fake birds 
% in at least five provinces 
\cite{china_drones}.
Shell recently launched a program based on the belief that smart drones can increase workplace safety and improve maintenance \cite{shell}, while vendors such as Amazon, DHL, and Alibaba have invested into UAVs-aided mail delivery and cargo transport \cite{amazon, dhl, alibaba}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \textbf{COMPLETELY MOTIVATE THE NEED OF CREATING A FULLY PROGRAMMABLE WIRELESS MESH NETWORK OF UAV + SDR}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Use in networking
Outside the numerous military and civil applications, UAVs especially attracted the attention of the wireless networking community.
% , where UAV-aided communications is a fast emerging topic.
Thanks to their inherent autonomy of operations, high mobility, processing power, and reduced size, UAVs are expected to be involved in numerous present and future IoT-related applications \cite{gupta2016survey}.
% , where their relatively low cost and high flexibility can be a key enabler towards new generations wireless networks 

% It is widely believed that integrating the current terrestrial architecture with new generations UAVs wireless networks can help shaping the future of wireless network infrastructure, both in relieving ground infrastructure congestion with smart offloading and in fast service recovery in case of unexpected damage or disaster scenario \cite{gupta2016survey}.

% drone features
%Given their ability to be operated autonomously, their high mobility, and their communication and processing power, Unmanned Aerial Vehicles (UAVs) are expected to be involved in numerous IIoT-related applications, where multimedia and video streaming plays a key role
%In view of their relatively low cost and high mobil- ity, unmanned aerial vehicles (UAVs) have recent- ly found applications in areas other than those related to the military and reconnaissance
%This is one of the few promising projects proposed in the recent past that can potentially pave the way in exploiting drones as vehicles of communication for future wireless net- works
%However, in unexpected or emergency situations (such as disaster relief and service recovery), the deployment of terres- trial infrastructures is economically infeasible and challenging due to high operational expenditure as well as sophisticated and volatile environments.  

% network applications
%UAV-aided communication is an emerging topic in the field of next generation networks. It is widely believed in academia that UAVs can help shape the public safety networks of the future, whereby drones, due to their greater mobility, may provide fast service recovery in the event of network infrastructure being damaged. Even if such a scenario does not arise, UAVs may contin- ue to relieve network congestion as their inclusion in the network would allow base stations (BSs) to offload some of the latter’s cellular traffic to the former. 
%Facebook (called Aquila) aims to use swarms of drones to provide “WiFi in the sky” service to remote areas.
%A good example is an Industry 4.0 factory premises equipped with indoor drones (e.g., for moving accessories) controlled by software components running in the cloud (local or remote).
%SDN, NFV and SFC are key enablers of future network services and applications, and they are essential building blocks of 5G systems. 



% UAV use and applications
%Unmanned Aerial Vehicles (UAVs) are autonomous aircrafts without the need of a pilot to be on board during the flight. UAV usage started with military applications, but now UAVs are getting more and more popular for public, civil, and even personal appli- cation military use cases, UAVs are deployed to execute military operations, such as battlefield inspection, geographic map- ping of inaccessible terrain, border control surveillance, etc. On the other hand, in public and civil use cases, UAVs can be used by in- dividuals or companies for aerial photography, video surveillance, etc. 
%To handle this issue, intelligent het- erogenous architecture by leveraging unmanned aerial vehicles (UAVs) (or commonly known as drones) [3] has been consid- ered to be a promising new paradigm to facilitate three central usage scenarios of future wireless networks, i.e., enhanced mobile broadband (eMBB) with bandwidth-consuming, ultra- reliable low-latency communication (URLLC) and massive machine-type communications (mMTC). 
%In particular, UAV-aided eMBB can be regarded as an important complement to the 5G cellular networks 
%As a result, UAVs are identified as an important component of 5G/B5G wireless technologies.
%Drones, also known as unmanned aerial vehicles (UAVs), have been used mainly in military applications for many years. However, there has been a recent increase in the use of UAVs in non-military fields, which is inspired by the 5G revolution. 
%Such fields include precision agriculture, security and surveillance, delivery of goods, and provisioned services
%Owing to the versatility and high mobility of UAVs, low- altitude UAVs are extensively used in diverse fields for differ- ent applications and purposes. On the standpoint of wireless communication aspects, UAVs can be employed as aerial communication platforms (e.g., flying base stations (BSs) or mobile relays) by mounting communication transceivers to provide/enhance communication services to ground targets in high traffic demand and overloaded situations, which is commonly referred to as UAV-assisted communications [5]– [9]. On the other hand, UAVs can also be used as aerial nodes to enable a multitude of applications ranging from cargo delivery to surveillance, which is commonly referred to as cellular-connected UAVs
%      In most current contexts, UAVs are equipped with communication devices or dedicated sensors that can enable a myriad of applications such as low altitude surveillance, post-disaster rescue, logistics application and communication assistance.
%   In recent years, the advancement of low-cost com- ponents and open source auto-pilot software stacks (MultiWii, LibrePilot, APM, and Pixhawk) have dra- matically reduced the unit cost of making drones. As a result, UAVs have become widely accessible to other industries and have opened up opportunities for tech- nological advancement. For example, in the telecom- munication industries, UAVs have been of great help in accomplishing site survey tasks to tackle latent prob- lems in cellular networks such as inference reduction and load balancing    
% The key driver of UAV networking is that UAVs can be used for autonomous flights, either by following a-priori flight missions or through the aid of more complex dynamic automation systems, coordinating a swarm-network.   

While the wireless capability of most of the UAV is somehow limited to Wi-Fi, housing an on-board Software Defined Radio (SDR) has been successful to extend their networking functionalities. 
This is possible thanks to the newer SDR, which are smaller and lighter, and efficiently interface with the compute board over USB without requiring any additional power.

% EXTENDING WIRELESS FUNCTIONALITIES
Extending wireless functionalities helps in cooping with inflexible network cards, that are not capable of keeping up with the quickly evolving pace of wireless standards, nor of adopting application-specific protocol designs, mainly due to their limited programmability and re-configurability. 
Furthermore, inflexible network cards are not well-suited to provide long-range connectivity among mobile UAVs.

On the contrary, 
employing a fully re-configurable radio platform, it is possible to provide tangible solutions to a plethora of UAV networking problems involving network coverage, security, spectrum-efficiency and interference management.


% Being able to reconfigure the RF front-end allows real-time frequency selection based on UAV location and channel conditions or modulation reinforcement or frequency switch reacting to selective-frequency jammers attacks  (or high interference scenarios).
% Similarly, SDRs and UAVs can be used in synergy to implement location-aware cognitive radio applications where the swarm detects and uses white spaces available at different locations of the deployment area.

% The above discussion shows that by relying upon legacy and inflexible RF front-ends will result in poor performance and connectivity outages. On the contrary, a fully re-programmable SDR-based swarm might be able to self-adapt to continuously changing channel and mobility conditions, thus always attaining the best performance in terms of efficiency, connectivity and security.

%%%%%%%%%%%%%%
% SDR can be employed alongside with on-board network card, which are effective to guarantee high transmission rates, but they are not well-suited to provide long-range connectivity among UAVs. 
% UAVs far away one from another might not be able to communicate through standard WiFi links, thus calling for systems that provide long-range connectivity through low frequency transmissions (e.g., UHF/VHF).

% Therefore, deploying new protocols or standards is prohibitive in terms of both cost and time on traditional network cards.At the same time, application-specific (e.g. CR, QoS-constrained battlefield operations, and aviation signaling) and context-specific (cargo delivery) protocol designs require a more flexible and reconfigurable wireless infrastructure.


% The advantage of a SDR-enabled communications in swarms of UAVs is not only limited to prototyping aspects. 
% On the contrary, by relying on a fully programmable platform, it is possible to provide tangible solutions to a plethora of UAV networking problems involving network coverage, security, spectrum-efficiency and interference management.

% A major challenge with swarms of flying vehicles, is how to ensure reliable and continuous connectivity among UAVs.
% They move fast and they might be located far away one from another. 


% ***WiFi cards that are mounted on the majority of commercially-available UAVs are effective to guarantee high transmission rates, but they are not well-suited to provide long-range connectivity among UAVs. 
% ***Accordingly, two UAVs far away one from another might not be able to communicate through standard WiFi links, thus calling for systems that provide long-range connectivity through low frequency transmissions (e.g., UHF/VHF). 







% in the case of malicious attackers such as jammers (or high interference scenarios), being able to reconfigure the RF front-end makes it possible to rapidly switch to those frequencies that are not jammed (or in general with better SINR values)
% The unique feature of SDRs is the possibility to (1) have both high-data rate WiFi communications and long-range communications on the same hardware; and (2) select which frequency to use in real-time according to current positions of UAVs and channel conditions.
 
% Furthermore, in the case of malicious attackers such as jammers (or high interference scenarios), being able to reconfigure the RF front-end makes it possible to rapidly switch to those frequencies that are not jammed (or in general with better SINR values), and to adopt modulation schemes that are more robust and resilient to interference and jamming signals.
% Similarly, SDRs and UAVs can be used in synergy to implement location-aware cognitive radio applications where the swarm detects and uses white spaces available at different locations of the deployment area.



% Ever since the introduction of Software defined Radio (SDR), the research community has produced advanced wireless networking technologies with run-time re-configuration and software programmability at different layers of the protocol stack.
Despite most of the research efforts in the last years employed SDR-based experimental infrastructures, only few of them worked toward a self-optimizable 
% software-defined 
reconfigurable wireless network spanning across all the layers of the protocol stack [XX]. 
This is even more true for UAV-based SDR applications, where most of the works limit their SDR-based architecture efforts to solely testbed prototyping [XX].


While alluring to the several benefits the future networks can take advantage of, the UAV/SDR paradigm has suffered almost invariably from the lack of adequate and coherently designed abstractions to control it.
% (i) define, with a structured methodology, overall network behavior spanning across all layers of the protocol stack and motion control;
% (ii) define distributed decision-making algorithms to control such interactions to work at single nodes of the network, independently. 
Thus, even essential networking functionalities and motion control often need to be manually controlled for every individual network control problem.








% lacking of a centralized control architecture.

% needs
%UAVs can be used for autonomous flights, either by following preprogrammed flight plans or through the help of more complex dynamic automation systems. 
%Therefore, an intelligent inter-UAV coordination protocol must be defined to control the behaviors of multiple UAVs, maximizing the benefits of a UAVNet.
%Furthermore, to support broadband wireless communications in a large geographical area, a swarm of UAVs forming Flying Ad Hoc Networks (FANETs) [12], [13] and establishing connection links with the ground nodes, have been studied theoretically and validated through field experiments
%A swarm of UAVs are capable of forming scalable multi-UAV networks and offering ubiquitous connectivity to ground users. Benefiting from its high flexibility and rapid provision features, the multi-UAV network is a feasible solution to recover and expand communication in fast and effective ways.    
%Some early efforts have been dedicated to heterogeneous networks (HetNets) (i.e., deploy various small cells) to meet these growing demands



% \item Present the problem: how to control a network consisting of a large number of nodes, with coupled behavior, easily and autonomously. recall that the swarm is unrealiable and time-varying, connection is not always guaranteed.

% While alluring to the several benefits that future networks can benefit from, the road toward incorporated UAVs and wireless networks is not without challenges.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \textbf{LIMITS OF CURRENT SDN FOR WIRELESS}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Since its introduction, traditional architectures started investing into Software Defined Networking to address the previously mentioned challenges. However, SDN have not found their way into distributed wireless networks yet.

Despite its success in addressing the mentioned challenges in traditional networks, Software Defined Networking has not found its way into distributed wireless networks yet.
Besides the lack of a centralized network control architecture, separating control and data plane in UAV wireless networks face some severe challenges.
Mobility patterns and protocol stack parameters
% physical layer parameters, MAC state and routing decisions 
are inherently coupled in a wireless infrastructure-less flying environment. 
3D-mobility, node unreliability, volatile network state, critical power usage,
% strictly regulated operations, 
and unique tasks such as remote sensing missions or ground network assistance, pose even more serious challenges to the design of a distributed, state-less control framework for UAV wireless networks. 



%A reliable communication infrastructure among the UAVs becomes critical in maintaining this connected network for the data relaying tasks. However, traditional protocols and algorithms responsible for end-to-end (e2e) operation do not fully meet the challenges of the dynamic environments where UAVs operate

%This UAV controlling protocol manages both the inter-UAV communication (i.e., routing protocols), as well as the UAV movement trajectory. In this context, Software-Defined Networking (SDN) [8–10] is a promising approach for this multi-UAV controlling task, since it introduces complete network programmability by separating the control plane and data plane.  




%SDN has been successfully applied in wired networks, such as data center networks or backbone networks. Specifically, these net- works have a centralized architecture, where a control center is responsible for network management [11]. The SDN controller is deployed in the control center, and it is aware of the global net- work conditions to optimize the network operations, by dynami- cally configuring the data plane routes
%For SDN deployments in wired networks with fixed infrastructure topology, programmabil- ity means that the control plane adaptively adjusts the data path, and the data plane follows the instructions to forward the packet through different interfaces. 
%On the other hand, SDN applied to UAVNets, the UAV programmability means to control the mobility trajectory of the UAVs in order to avoid UAV collisions or to im- prove the application performance, to determine the data routing paths, to change the packet transmission parameters (data rate or transmission power) due to performance or energy reasons, and others. 

%UAVNets are mostly deployed to perform specific tasks, such as assisting disaster recovery communications, surveillance monitoring, remote sensing/searching, etc. In these tasks, UAVNet nodes must collaborate with each other and their behaviors (both the data transmission and the UAV movement) should be con- trolled by a centralized entity, i.e., a controller






%A reliable communication infrastructure among the UAVs becomes critical in maintaining this connected network for the data relaying tasks. However, traditional protocols and algorithms responsible for end-to-end (e2e) operation do not fully meet the challenges of the dynamic environments where UAVs operate



%UAVs can be used for autonomous flights, either by following preprogrammed flight plans or through the help of more complex dynamic automation systems. Therefore, an intelligent inter-UAV coordination protocol must be defined to control the behaviors of multiple UAVs, maximizing the benefits of a UAVNet. This UAV con- trolling protocol manages both the inter-UAV communication (i.e., routing protocols), as well as the UAV movement trajectory. In this context, Software-Defined Networking (SDN) [8–10] is a promising approach for this multi-UAV controlling task, since it introduces complete network programmability by separating the control plane and data plane.

%SDN has been successfully applied in wired networks, such as data center networks or backbone networks. Specifically, these net- works have a centralized architecture, where a control center is responsible for network management [11]. The SDN controller is deployed in the control center, and it is aware of the global net- work conditions to optimize the network operations, by dynami- cally configuring the data plane routes
%For SDN deployments in wired networks with fixed infrastructure topology, programmabil- ity means that the control plane adaptively adjusts the data path, and the data plane follows the instructions to forward the packet through different interfaces. On the other hand, SDN applied to UAVNets, the UAV programmability means to control the mobility trajectory of the UAVs in order to avoid UAV collisions or to im- prove the application performance, to determine the data routing paths, to change the packet transmission parameters (data rate or transmission power) due to performance or energy reasons, and others. UAVNets are mostly deployed to perform specific tasks, such as assisting disaster recovery communications, surveillance monitoring, remote sensing/searching, etc. In these tasks, UAVNet nodes must collaborate with each other and their behaviors (both the data transmission and the UAV movement) should be con- trolled by a centralized entity, i.e., a controller.






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \textbf{NEED FOR A FRAMEWORK TO CONTROL IN A PROGRAMMATIC WAY MESH NETWORKING FUNCTIONALISTS AT ALL LAYERS OF PROTOCOL STACK PHY->TRANSPORT + FLIGHT }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Ultimately, the development of reconfigurable and programmable UAV wireless networks needs an intelligent framework 
% to control in a programmatic way UAV movements and mesh networking functionalities at all layers of the protocol stack. 
to provide the abstractions to
(i) define, with a structured methodology, overall network behavior spanning across all layers of the protocol stack and motion control;
(ii) define distributed decision-making algorithms to control such interactions to work at single nodes of the network, independently. 

% Ultimately, an intelligent control framework employing the SDR re-configurability and programmability  to  optimize the behavior of multiple UAVs is an undeniable need for the development of UAV-based networking.
Such framework will be a critical inter-UAV coordination mechanism, guaranteeing reliable communication, maintaining UAVs connected too each other, coordinating communication protocols, and handling network parameters at run-time.

% Such a framework not only has to ensure a reliable physical layer, preventing network isolation, provide feasible routing paths, and take care of ordinary network protocol functioning; 
Moreover, it must be self organizing, require little human intervention, and most importantly must be fast adapting to rapidly changing UAV network conditions.
% It must allow the flexibility to define a wide range of control features, selecting protocols, imposing network QoS requirements, and node-specific constraints. 
% In conclusion, the control framework operations have to extend beyond traditional control techniques, enabling high-level network control, yet running on distributed devices; hiding low-level infrastructure details to the controller, yet allowing single node constraints. 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \textbf{PHILOSOPHY:
% DEFINE ON A HIGH LEVEL CENTRALIZED ABSTRACTION 
% PRESENT MATHEMATICALLY 
% DECOMPOSE VERTICALLY + HORIZONTALLY 
% EXECUTE ABSTRACT REPRESENTATION
% PPS}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this article, we propose SwarmControl, a softwarized framework applying the basic principles of SDN, distributed optimization, and control problem decomposition to UAV networking; aiming to provide software programmability to the network parameters and motion control.
% resume SwarmControl
SwarmControl hides the details of the network infrastructure to the network controller and provides them with a high-level network abstraction and control APIs, based on which, they can dictate the overall network behavior with no required knowledge of the low-level network implementation details.
% Most importantly, SwarmControl will define a mathematical representation of the centralized network control problem based on the controller's input. 
% From the network control problem, SwarmControl will automatically generate a set of independent distributed network control algorithms to be executed at individual UAVs of the network, yet not revealing the distributed implementation of the network control operations to the controller.
The contribution of the article can be summarized as follows:
\vspace{-2mm}
\begin{itemize}
    \item \textbf{SwarmControl architecture design}:
    We propose SwarmControl two-module design for UAV wireless networks:
    (i) Central Control Framework, 
    and (ii) Programmable Protocol Stack.
    % Each of the two modules employs three sub-modules:
    % Control Panel, Problem construction, and  Problem Decompositixon; Control Plane,  Register Plane, and Data Plane; respectively.
    \item \textbf{Control problem definition and decomposition for UAV-Net}: 
    We employ well-studied notions of network abstraction and consolidated automatic control problem decomposition principles and rigorously extend them to UAV-swarm networks, to first construct a centralized network control problem based on controller's network behavior goal, and then decompose it into distributed algorithms to be run at single UAV nodes of the network.
    % We show the foundations of SwarmControl Central control Frameworks problem construction and distributed decomposition as solid and based on UAV-Net adaptation of well studied network abstraction techniques and consolidated control problem decomposition principles.
    \item \textbf{SwarmControl Programmable Protocol Stack (SC-PPS)}:
    The distributed solution algorithms run at single nodes, distributively communicate with each other.
    To accomplish that, we developed an all-new general purpose SwarmControl Programmable Protocol Stack (PPS) spanning across 
    all the networking protocol layers and the motion domain.
    Basing our layout on SDN founding principles, we designed SwarmControl PPS following a three plane structure: (i) control plane, (ii) register plane, and 
    (iii) data plane.
    % , tightly but independently interacting with each other, covering all the protocol layers together with the motor control.
    \item \textbf{Prototyping and assessment}:
    We implemented SwarmControl functionalities at a network control host.
    Employing the newly designed PPS, we assessed the performances of our automated distributed solution approach on a multi-hop 8-UAV/SDR flying network, whose nodes we first prototyped and then deployed. 
\end{itemize}


%In this article, we propose a Software-Defined UAVNet archi- tecture (SD-UAVNet), which implements the concept of SDN into UAVNets to separate the control and data plane, as well as to pro- vide network programmability by controlling UAVs’ operation pa- rameters. With the proposed SD-UAVNet architecture, we focus on the problem of optimal UAV relay node placement for real-time video services, which reduces the impact of node mobility on the QoE of delivered videos. The SD-UAVNet controller considers the global UAV context information to prevent UAV collisions, optimize the UAVs’ movements, and establish a routing path that determines the relay node deployment to provide video transmission with QoE support. Specifically, the controller considers multiple UAV context information for routing and UAV placement decisions, namely, UAV positions, UAV movement trajectories, and residual energy.




% \item gains we achieve 
% We tested SwarmControl effectiveness and flexibility performances compared with the state of the art and other optimization frameworks in different scenarios, network deployments and configurations. 
% We proved the proposed control framework effectiveness for stand-alone aerial wireless networks as well as for mixed ground/aerial infrastructures, achieving an average throughput gain of XX when applying performance maximization control problems, and XX overall power savings when we apply energy saving control problems.

% \item structure 
The article is organized as follows:
In Section \ref{sec:design}, we present a design overview of SwarmControl, and describe the network abstraction principles in Section \ref{sec:ncp}. 
We discuss the distributed algorithm generation approach in Section \ref{sec:distributed}, and describe the SwarmControl PPS design in Section \ref{sec:pps}.
We present the framework evaluation in Section \ref{sec:evaluation}, discuss limitations and future work in Section \ref{sec:discussion}, and finally we draw the main conclusions in Section \ref{sec:conclusion}.

\begin{figure}[t]
% \centering
\includegraphics[width=0.48\textwidth]{Figures/SwarmControl_sys_v1.pdf} \vspace{-3mm}\caption{ \small SwarmControl Architecture.}\vspace{-5mm}
\label{fig:arch}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%3/15/2019%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Introduction}
\label{sec:introduction}
Radio access networks will soon be expected to support up to a 1000-fold increase in traffic volumes and 100 billion ubiquitously connected wireless devices, all with heterogeneous requirements in terms of data processing, battery lifetime, transmission range, and latency [XX].
This will exert extraordinary pressure on the current infrastructure, in terms of high capacity and scalability demands.
To address these issues, intelligent unmanned aerial vehicles (UAVs, or drones) are a promising technology to extend the infrastructure of future wireless networks and to make it more flexible [XX].

Swarms of UAVs have been proposed for a variety of military applications spanning battlefield inspection, geographic mapping of dangerous terrains, border control, and aerial surveillance.
For example, at least 30 military and government agencies in China have strengthened their surveillance network with small drones resembling birds \cite{china_drones}.
Similarly, US Army soldiers will be equipped with nano drones to obtain augmented and accurate information about their surroundings \cite{nano_drones}.
Only more recently UAVs have been employed in non-military applications. Indeed, public and civil organizations have started leveraging UAVs to provide innovative services in precision agriculture, emergency response, environmental monitoring, and delivery of goods. 
For example, Shell recently launched "Eye in the sky", a program where smart UAVs are equipped with gas sensors and cameras to enhance workplace safety conditions and facilitate maintenance operations \cite{shell}. Similarly, vendors such as Amazon, DHL, and Alibaba have invested into UAV-aided delivery of goods and cargo transportation \cite{amazon, dhl, alibaba}.

Besides the above applications, UAVs have also attracted the interest of the networking community as a ``tool'' to provide new capabilities to wireless networked systems.
Thanks to their unique features such as fast deployment, high mobility, processing capabilities, and reduced size, UAVs find application in numerous present and future IoT and 5G scenarios \cite{gupta2016survey}, as an example, to increase network coverage or to provide advanced and high-performance network services to mobile users. 

While alluring to the several benefits the future wireless networks can take advantage of, controlling UAV-Networks suffers from the exceptional challenges typical of a wireless flying environment.
% However, UAV-networks are still unexplored because of the exceptional networking challenges of a wireless flying environment.
Even basic networking functionalities such as network formation and point-to-point communication are threatened by unstable channel characteristics and fragile network connectivity.

Endowing drones with software defined radios (SDR) can help overcome the limitations of the on-board inflexible wireless interfaces (e.g., Wi-Fi). 
SDR front-end abstractions provide the programmability needed to keep up with the evolving pace of wireless standards and the re-configurability necessary to support the 
% diverse UAV applications, 
fragile open-sky UAV communications, 
impracticable over short-range interfaces such as Wi-Fi. 
In spite of the indisputable benefits of a re-configurable UAV/SDR-based infrastructure, most current research efforts have been limited to programmability of the SDR at the physical layer, while a comprehensive software-defined networking paradigm spanning all layers of the protocol stack is still to be developed. 

Without an adequate software-programmable control infrastructure, 
the network operator would have to construct a network control problem by manually defining variables, objectives, and constraints. Such an approach has several major drawbacks. 
First, controlling a swarm of UAVs asks for a deep understanding of the interactions between mobility and networking, and it often requires coding expertise to write hundreds or thousands of lines of code. 
Second, it is not well-suited for dynamic fast-changing environments, such as UAV-networks.
Finally, it relies on the assumption that the network operator is aware of low-level network infrastructure details and protocol implementations (e.g.,  UAVs location, their neighboring UAVs, their maximum tx power, tx modulation, and central frequency); an assumption that often does not hold. 
% This way controlling a UAV-netowork essential networking and motion functionalities often requires ad-hoc programming and manual tuning, which often requires coding expertise to write hundreds or thousands of lines of code. 
% The reasons behind such shortcoming are numerous. 
% Besides the lack of a centralized network control architecture, controlling a swarm of UAVs requires deep understanding of the interactions between mobility and networking. 

% SwarmControl aims at surpassing traditional control approaches developing an automated virtualized control framework for UAV networks requiring minimal NO intervention.
% SwarmControl automatically generates optimization control problems starting from few input lines of code, hiding the network infrastructure details and the distributed implementation to the NO.

% Ultimately, the development of reconfigurable and programmable UAV wireless networks needs an intelligent framework to:
% \textbf{(i) specify the desired network behavior;
% and 
% (ii) implement it by means of distributed control strategies spanning across all layers of the network protocol stack and motion control.}
% Such a framework is expected to implement a self-organizing and coordinated UAV-network that dynamically adapts to UAV locations and network state, and ultimately guarantees reliable communication and connectivity with minimal human-machine interactions.
Motivated by recent and growing interest in automated optimization theory, in this article we propose SwarmControl, a framework that attempts to combine the basic principles of SDN, distributed optimization, and control problem decomposition to mobile networks of UAVs. 
SwarmControl aims at providing network programmability through a high-level abstraction and control API that hides (i) low-layer network functionalities needed to obtain high-performance in mobile and dynamic environments; (ii) the distributed nature of  the network control problem; (iii) the interdependence between motion control and the network control problem.
With SwarmControl, the network ``operator'' can program the overall network behavior without a-priori knowledge of the network topology details, its mobility patterns, and details of the distributed control implementation.
Moreover, such a framework is expected to implement a self-organizing and coordinated UAV-network that dynamically adapts to UAV locations and network state, and ultimately guarantees reliable communication and connectivity with minimal human-machine interactions.

The main contributions of this paper can be summarized as follows:
\vspace{-0mm}
\begin{itemize}
    \item \textbf{SwarmControl framework}:
    We introduce SwarmControl, a novel softwarized and SDR-based control framework for UAV wireless networks. 
    % The architecture of SwarmControl is based on two main components, namely a {\em Central Control Framework} (CCF) and a {\em Programmable Protocol Stack} (PPS). XXX maybe we should change this name to differentiate from WNOS as this includes also the mobility part XXX
    SwarmControl employs notions of network abstraction and automatic control problem decomposition principles to provide an unified abstraction of the networking and flight domains, that enables the definition and the actuation of complex control problems.
    SwarmControl first constructs a centralized network control problem based on the desired behavior, and then decomposes it into distributed sub-problems to be solved at single UAVs;
    % These components are used, respectively, to automatically transform control directives specified by the network operator on a centralized high-level abstraction (CCF) into actuation strategies that are distributively implemented and involve joint control of the networking functionalities at all layers of the protocol stack (from physical to transport layer) and the motion domains;
    % \item \textbf{Control problem definition and decomposition for UAV-Net}: 
    % XXX here, I would rewrite saying that we propose an abstraction that enables definition of ...network control + flight control ... and decomposition into distributed bla bla bla XXX
    \item \textbf{SwarmControl Programmable Protocol Stack (SC-PPS)}:
    We develop a novel general purpose Programmable Protocol Stack (PPS) spanning across 
    all the networking protocol layers and the motion domain.
    Basing our layout on SDN founding principles, we designed SwarmControl PPS following a three plane structure: (i) decision plane, (ii) register plane, and (iii) data plane.
    The PPS executes the distributed solution algorithms generated by the Central Control Framework, and enforces the networking and motion strategies on each UAV;
    \item \textbf{Prototyping and assessment}:
    We prototype SwarmControl over Intel Aero Drones interfaced with Ettus B205mini-i SDRs. 
    Radios and drone flight are jointly controlled by the SwarmControl PPS installed on the drone's Intel compute board. 
    We assess the performance of SwarmControl on a 8-UAV/SDR multi-hop flying network and we compare them with other state-of-the-art solutions. 
    Our experiments show that SwarmControl effectively improves the network performance (up to $231\%$ of throughput gain) and dynamically adapts networking and motion strategies to different control problems and channel conditions.
\end{itemize}

The remainder of this paper is organized as follows:
In Section \ref{sec:design}, we present a design overview of SwarmControl architecture. 
We provide a detailed description of the network abstraction principles in Section \ref{sec:ccf}, 
% we discuss the distributed algorithm generation approach in Section \ref{sec:distributed}, 
and describe the SwarmControl PPS design in Section \ref{sec:pps}.
We present the framework evaluation in Section \ref{sec:evaluation}, and draw the main conclusions in Section \ref{sec:discussion}.

==> toy_example_backup.tex <==
subsection{Toy Example of UAV Network Control} 
\label{sec:example}
We consider a simple network of five UAV nodes as depicted in Fig.~\ref{fig:graph}, where two source nodes, $A$ and $B$, transmit toward a common destination $E$ via relay nodes $C$ and $D$.
Let the transmission range of each node $i\in\mathcal{N}=\{A,B,C,D,E\}$ depend on its transmission power $p_i$. 
We assume that the source nodes' transmission power is not enough to reach the destination $E$ and, based on routing polices, they independently employ a relay nodes $C$ and $D$, to forward their traffic toward the destination.
Let us consider the case where the network operator (NO) aims at maximizing the overall network throughput ($\texttt{max}\_\texttt{throughput}$) 
via optimizing the transmission rate, routing tables, power allocation, and UAV locations.
The NO also specifies node-specific constraints to $A$, $B$ and $E$, forced in "hold mode", i.e., they are instructed to keep their initial location unchanged,  while $C$ and $D$ are let free to move.
% The impact of mobility on the relaying tasks is threefold: 
% (1) the UAVs can move to get closer to the source and destination, and thus improve the signal-to-interference-plus-noise ratio (SINR) along the session path; 
% (2) getting closer to other nodes might result in increased mutual interference and degrade the overall network performance; 
% and (3) moving outside the transmission range of other UAVs may result in network partitioning. 

Before going through the automated network control construction process, let us introduce some notation.
Let $r_i, i\in\mathcal{N}$ represent the session rate of each node, with $r_E=0$ and $x_{kn}\in\{0,1\}$ be the routing strategy of source nodes where $k\in\{A,B\}$ and $n\in\{C,D\}$. Specifically, $x_{kn}=1$ if source node $k$ routes its traffic through relay node $n$, and $x_{kn}=0$ otherwise. 
Finally, the location of each node $i\in\mathcal{N}$ is denoted as $\pi_i$, and since source nodes can only select one relay at a time, we have $x_{kC}=1-x_{kD}$. 

As mentioned in Section \ref{sec:ncp}, SwarmControl processes the control directives of the network operator and, by relying on a UAV network abstraction, constructs the following optimization problem:
\textbf{[XX here the problem must be general, not specific to the example XX]}
\begin{align}
\underset{\mathbf{r},\mathbf{x},\mathbf{p},\boldsymbol{\pi}}{\text{maximize}} \hspace{0.2cm} & r_C + r_D, \label{prob:cap:ut} \\
\text{subject to} \hspace{0.2cm} & r_C \leq x_{AC} r_A + x_{BC} r_B,   \label{prob:cap:c1} \\
                                 & r_D \leq (1 - x_{AC}) r_A + (1 - x_{BC}) r_B,   \label{prob:cap:c2} \\
                                 & \mathrm{SINR}_{kC}(\mathbf{p},\boldsymbol{\pi}) \geq x_{kC} \gamma, \hspace{0.25cm} \mbox{ for } k = A,B,  \label{prob:cap:c3} \\
                                 & \mathrm{SINR}_{kD}(\mathbf{p},\boldsymbol{\pi}) \geq (1 - x_{kC}) \gamma, \hspace{0.25cm} \mbox{ for } k = A,B,  \label{prob:cap:c4} \\                         
                                 & \mathrm{SINR}_{nE}(\mathbf{p},\boldsymbol{\pi}) \geq \gamma, \hspace{0.25cm} \mbox{ for } n = C,D,  \label{prob:cap:c5}
\end{align}
\noindent
where $\mathbf{r}=
\{r_A,r_B,r_C,r_D\}$, $\mathbf{x}=\{x_{AC},x_{BC}
\}$, $\mathbf{p}=\{p_A,p_B,p_C,p_D\}$, $\boldsymbol{\pi}=\{\pi_C,\pi_D\}$;
$\gamma$ represents the minimum SINR level to correctly decode received messages; and $\mathrm{SINR}_{kn}(\mathbf{p},\boldsymbol{\pi})$ represents the SINR experienced by node $n$ when receiving useful signals from node $k$. 
For example, if $k=A$ and $n=C$, $\mathrm{SINR}_{kn}(\mathbf{p},\boldsymbol{\pi})$ is defined as
% \begin{equation}
    $\mathrm{SINR}_{AC}(\mathbf{p},\boldsymbol{\pi}) = \frac{G(\pi_A,\pi_C)p_A}{N+G(\pi_B,\pi_C)p_B}$,
% \end{equation}
% \noindent
with $N$ being the ambient noise power and $G(\pi_k,\pi_n)$ being the channel coefficient between two nodes $k$ and $n$. In this  example, we assume that all nodes are in line-of-sight conditions and $G(\pi_k,\pi_n)$ can thus be computed through the free-space path loss model. 
Specifically, we have $G(\pi_k,\pi_n) = M d^{-\eta}(\pi_k,\pi_n)$, where $M$ is a positive constant, $\eta$ represents the path-loss coefficient, and $d(\pi_k,\pi_n)$ is the distance between position $\pi_k$ and $\pi_n$.
It is worth mentioning that, in reality, SwarmControl generates a problem with many more constraints to ensure the feasibility of the NCP. 
% Among others, SwarmControl includes a capacity constraint such that the transmission rate $r_i$ does not exceed the link capacity. 
For the sake of illustration we have deliberately omitted these additional constraints from Problem \eqref{prob:cap:ut}-\eqref{prob:cap:c5}, which however are also decomposed and treated as follows.

% Based on the constructed centralized NCP, the decomposition process starts.
First, SwarmControl detects optimization variables and classifies their coupling with the aid of the layered coupling graph introduced in Section \ref{sec:distributed}. 
A portion of the layered coupling graph generated by SwarmControl for this specific example scenario is illustrated in Fig. \ref{fig:graph}. 
For example, the transport layer transmission rate variables $r_A$ and $r_C$ are coupled through the link rate constraint \eqref{prob:cap:c1}.
Similarly, physical layer variable $p_A$  (node A) and the motion layer variable $\pi_{AC}$ (node C) are coupled through the physical link capacity constraint expressed in~\eqref{prob:cap:c3}.

Among others, while the lienar coupling between $r_C$ and $r_A$ in \eqref{prob:cap:c1} can be removed by using functions with separable variables, $r_A$ and $x_{AC}$ stronger nonlinear relationship in \eqref{prob:cap:c3} requires more complex decomposition tools such as partial linearization \cite{scutari2014decomposition}, Taylor series linearization, and Lagrangian duality \cite{gao2013duality}.
% additional efforts in the decomposition process. 
% In Fig. \ref{fig:graph} we provide a visual representation of horizontal (weak) and strong (vertical) couplings among NCP optimization variables.
% By using the above techniques, SwarmControl decomposed the NCP 
% , such as Lagrangian duality \cite{gao2013duality}, 
% separates NCP variables 
% and generates a set of independent sub-problems that can be solved through a series of distributed single-domain algorithms. 
% For the sake of illustration, and because of space limitations, 
We now showcase the decoupling process of Constraint \eqref{prob:cap:c3} for $k=A$ as an example. 
The remainder of Problem \eqref{prob:cap:ut}-\eqref{prob:cap:c5} can be decomposed similarly.
% Now we showcase the decomposition process taking Constraint \eqref{prob:cap:c3} with $k=A$ as an example, while the remaining expressions in Problem \eqref{prob:cap:ut}-\eqref{prob:cap:c5} can be decomposed similarly.
Following the definition of $\mathrm{SINR}_{kn}$, we can rewrite Constraint \eqref{prob:cap:c3} as 
\begin{align} \label{eq:example:1}
    \theta(\pi_C,p_A,x_{AC},p_B) = & \nonumber \\
    G(\pi_A,\pi_C)p_A  - x_{AC} \gamma N - & x_{AC} \gamma G(\pi_B,\pi_C) p_B \geq 0
\end{align}
\noindent
with optimization variables  $\pi_C,p_A,x_{AC}$ and $p_B$. 
Optimization variables at different UAVs and at different layers of the protocol stack are coupled together by the nonlinear relationships in \eqref{eq:example:1}.
Given that a generic function $f(x,y)$ can be linearized by using its first-order Taylor expansion at any point $(a,b)$ as
\begin{equation} \label{eq:example:2}
    f(x,y) \!\!\approx\!\! f(a,b)\! + \!\left. \frac{\partial f(x,y)}{\partial x} \right|_{a,b}\!\!\!\! (x-a)\! + \!\left. \frac{\partial f(x,y)}{\partial y} \right|_{a,b}\!\!\!\! (y-b) 
\end{equation}
and applying the same principle to \eqref{eq:example:1}, we first (i) generate a linearized constraint, and then (ii) use Lagrangian duality to include the linearized constraint into the objective function of Problem \eqref{prob:cap:ut}-\eqref{prob:cap:c5}. 
Being $\tilde{\theta}(\pi_C,p_A,x_{AC},p_B)$ the linearized version of \eqref{eq:example:1}, we can generate the following Lagrangian dual function 
\begin{equation} \label{eq:example:3}
    % L(r_C,r_D,\pi_C,p_A,x_{AC},p_B,\lambda_A)
    L\!=\! r_C + r_D + \lambda_A \tilde{\theta}(\pi_C,p_A,x_{AC},p_B)
\end{equation}
\noindent 
where $\lambda\geq0$ is the Lagrangian multiplier associated to the linearized constraint \eqref{prob:cap:c3}. 
The dual function $L$ in \eqref{eq:example:3} is now formulated with separable variables with respect to $(r_C,r_D,\pi_C,p_A,x_{AC},p_B)$, with only $\lambda_A$ keeping track of the previous coupling.  \textbf{[XX meaning what? XX]}
By extending the above decomposition procedures to the whole NCP \eqref{prob:cap:ut}-\eqref{prob:cap:c5} this can be decomposed into multiple independent sub-problems.

The obtained sub-problems are then solved through numerical solution algorithms, where the optimization variables and network parameters are represented through textual keywords.
\begin{figure*}[t]
\centering
\includegraphics[width=0.7\textwidth]{Figures/PPS_v4.pdf} \vspace{-0mm}\caption{ \small  Drone Programmable Protocol Stack Prototype.}
\vspace{-0mm}
\label{fig:PPS}
\end{figure*} 
For example, let us consider the term $G(\pi_k,\pi_n)p_k$ at the numerator of the SINR expression previously defined. 
This term is transformed into the string $\texttt{CCGAINDEST}*\texttt{txpower}$ and interpreted through the SwarmControl protocol library available at the network nodes Drone Programmable Protocol Stack (Drone PPS). 
In this case, representing $\texttt{CCGAINDEST}$ the channel gain coefficient with the next hop, it is replaced with its real-time value available at the Drone PPS.
Similarly, for optimization variables such as the transmission power ($\texttt{txpower}$), the library indicates that the keyword is to be used as an input of the optimization solver.
The generated scripts will then be distributed and executed at individual UAVs in the Drone PPS.
